An Approach to Regular Separability in Vector Addition Systems

We study the problem of regular separability of languages of vector addition systems with states (VASS). It asks whether for two given VASS languages K and L, there exists a regular language R that includes K and is disjoint from L. While decidability of the problem in full generality remains an open question, there are several subclasses for which decidability has been shown: It is decidable for (i) one-dimensional VASS, (ii) VASS coverability languages, (iii) languages of integer VASS, and (iv) commutative VASS languages. We propose a general approach to deciding regular separability. We use it to decide regular separability of an arbitrary VASS language from any language in the classes (i), (ii), and (iii). This generalizes all previous results, including (iv).

==> general.tex <==
% !TEX root = main.tex

\wojtek{This should be defined earlier}
Let $L$ and $K$ be languages. We write $\sep{L}{K}$ if there is a regular $R$ with
$L\subseteq R$ and $R\cap K=\emptyset$. For a rational transduction
$T\subseteq \Sigma^*\times\Gamma^*$, we define 
\begin{align*}TL=\{v\in\Gamma^* \mid \exists (u,v)\in T,~u\in L\}, && T^{-1}=\{(v,u)\in\Gamma^*\times\Sigma^* \mid
(u,v)\in T\}. \end{align*}

\begin{lemma}\label{movetrans}
Let $T$ be a rational transduction. Then $\sep{L}{TK}$ if and only if $\sep{T^{-1}L}{K}$.
\end{lemma}
\begin{proof}
Suppose $L\subseteq R$ and $R\cap TK=\emptyset$ for some regular
$R$. Then clearly $T^{-1}L\subseteq T^{-1}R$ and $T^{-1}R\cap
K=\emptyset$. Therefore, the regular set $T^{-1}R$ witnesses
$\sep{T^{-1}L}{K}$. Conversely, if $\sep{T^{-1}L}{K}$, then
$\sep{K}{T^{-1}L}$ and hence, by the first direction,
$\sep{(T^{-1})^{-1}K}{L}$. Since $(T^{-1})^{-1}=T$, this reads
$\sep{TK}{L}$ and thus $\sep{L}{TK}$.
\end{proof}


We sometimes want to reduce the question of whether $\sep{L}{K}$ to
the question of whether $\sep{h(L)}{h(K)}$ for some morphism $h$.  Of
course, if $h^{-1}(h(K))=K$, then this follows easily from
\cref{movetrans}. Indeed, then $\sep{L}{K}$ iff $\sep{L}{h^{-1}(h(K))}$ iff $\sep{h(L)}{h(K)}$.
Let us show that it suffices that
$h^{-1}(h(K))\cap R=K\cap R$ for some regular superset $R$ of $L$.
\begin{lemma}\label{morphic-image}
  Let $L,K\subseteq\Sigma^*$ and $h\colon \Sigma^*\to\Gamma^*$ be a
  homomorphism.  If there is a regular $R$ with $L\subseteq R\subseteq
  \Sigma^*$ such that $h^{-1}(h(K))\cap R=K\cap R$, then $\sep{L}{K}$ if and
  only if $\sep{h(L)}{h(K)}$.
\end{lemma}
\begin{proof}
  $\sep{L}{K}$ iff $\sep{L\cap R}{K}$ iff $\sep{L}{K\cap R}$ iff
  $\sep{L}{h^{-1}(h(K))\cap R}$ iff $\sep{L\cap R}{h^{-1}(h(K))}$ iff
  $\sep{L}{h^{-1}(h(K))}$ iff $\sep{h(L)}{h(K)}$.\georg{Explain why every step is trivial or follows from \cref{movetrans}.}
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> picture-amalgamation.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,439); %set diagram left start at 0, and has height of 439

%Shape: Axis 2D [id:dp07743782245391018] 
\draw  (49,412) -- (611,412)(49,26) -- (49,412) -- cycle (604,407) -- (611,412) -- (604,417) (44,33) -- (49,26) -- (54,33)  ;
%Straight Lines [id:da9873120956449528] 
\draw [line width=1.5]    (228,339) -- (330,324) ;


%Straight Lines [id:da401857101829619] 
\draw [line width=1.5]    (125,387) -- (228,339) ;


%Curve Lines [id:da9584853971771883] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]    (145,302) .. controls (185,272) and (137,325) .. (177,295) ;


%Straight Lines [id:da7684944719137352] 
\draw [line width=1.5]    (177,295) -- (280,247) ;


%Curve Lines [id:da8314341722767573] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]    (280,247) .. controls (320,217) and (219,249) .. (259,219) ;


%Straight Lines [id:da9007653153761256] 
\draw [line width=1.5]    (259,219) -- (361,204) ;


%Curve Lines [id:da2753291638973735] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]    (361,204) .. controls (401,174) and (340,269) .. (380,239) ;


%Curve Lines [id:da05044856230576078] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (157,278) .. controls (197,248) and (146,255) .. (186,225) ;


%Straight Lines [id:da7446755620932114] 
\draw [line width=1.5]    (186,225) -- (289,177) ;


%Curve Lines [id:da42514340807928896] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (289,177) .. controls (329,147) and (314,203) .. (354,173) ;


%Straight Lines [id:da5422339135037434] 
\draw [line width=1.5]    (354,173) -- (456,158) ;


%Curve Lines [id:da949056723932101] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (456,158) .. controls (496,128) and (396,265) .. (436,235) ;


%Curve Lines [id:da74561882940504] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]    (177,193) .. controls (217,163) and (169,216) .. (209,186) ;


%Curve Lines [id:da5833422097376669] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (209,186) .. controls (249,156) and (198,163) .. (238,133) ;


%Straight Lines [id:da5824434354138336] 
\draw [line width=1.5]    (238,133) -- (341,85) ;


%Curve Lines [id:da1081077377359787] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]    (341,85) .. controls (381,55) and (280,87) .. (320,57) ;


%Curve Lines [id:da03505038767190838] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (320,57) .. controls (360,27) and (345,83) .. (385,53) ;


%Straight Lines [id:da9237355072843183] 
\draw [line width=1.5]    (385,53) -- (487,38) ;


%Curve Lines [id:da6952022164490457] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]    (487,38) .. controls (527,8) and (466,103) .. (506,73) ;


%Curve Lines [id:da7947152440401817] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (506,73) .. controls (546,43) and (446,180) .. (486,150) ;


%Straight Lines [id:da7286895788248409] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (145,302) -- (125,387) ;


%Straight Lines [id:da5141697313272611] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (157,278) -- (125,387) ;


%Straight Lines [id:da7737819450435529] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (177,193) -- (145,302) ;


%Straight Lines [id:da9331119759188556] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (177,193) -- (157,278) ;


%Straight Lines [id:da11715759422432148] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (380,239) -- (330,324) ;


%Straight Lines [id:da8134616148718465] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (486,150) -- (436,235) ;


%Straight Lines [id:da059548349426440494] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (436,235) -- (330,324) ;


%Straight Lines [id:da329945320736715] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (486,150) -- (380,239) ;


%Straight Lines [id:da8336670777886629] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (259,219) -- (228,339) ;


%Straight Lines [id:da04359366903142248] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (385,53) -- (354,173) ;


%Straight Lines [id:da264930039668387] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (354,173) -- (228,339) ;


%Straight Lines [id:da5377885836097857] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (385,53) -- (259,219) ;


% Text Node
\draw (196,375) node  [scale = 1.3][align=left] {$\rho$};
% Text Node
\draw (229,290) node  [scale = 1.3][align=left] {$\rho_1$};
% Text Node
\draw (202,236) node  [scale = 1.3][align=left] {$\rho_2$};
% Text Node
\draw (263,143) node  [scale = 1.3][align=left] {$\rho_3$};


\end{tikzpicture}


==> picture-runs.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,396); %set diagram left start at 0, and has height of 396

%Straight Lines [id:da7313518400507261] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (138,249) -- (103,281) ;


%Straight Lines [id:da5935269429215918] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (138,249) -- (151,340) ;
\draw [shift={(151,340)}, rotate = 81.87] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(138,249)}, rotate = 81.87] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da7461452257867053] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (138,249) -- (228,316) ;


%Straight Lines [id:da12563415872601913] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (244,273) -- (228,316) ;
\draw [shift={(228,316)}, rotate = 110.41] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(244,273)}, rotate = 110.41] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da1836638445355706] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (154,206) -- (244,273) ;


%Straight Lines [id:da06008915364510059] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (154,206) -- (138,249) ;


%Straight Lines [id:da49505511031975535] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (154,206) -- (103,281) ;
\draw [shift={(103,281)}, rotate = 124.22] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;

%Straight Lines [id:da4094822413422471] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (205,131) -- (154,206) ;
\draw [shift={(154,206)}, rotate = 124.22] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(205,131)}, rotate = 124.22] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da6228919663108438] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (256,56) -- (205,131) ;
\draw [shift={(205,131)}, rotate = 124.22] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(256,56)}, rotate = 124.22] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;

% Text Node
\draw[color={rgb, 255:red, 208; green, 2; blue, 27 }] (87,294) node  [scale=1.3][align=left] {$\pi$};
% Text Node
\draw[color={rgb, 255:red, 208; green, 2; blue, 27 }] (138,348) node [scale=1.3][align=left] {$\delta$};
% Text Node
\draw[color={rgb, 255:red, 208; green, 2; blue, 27 }] (230,330) node [scale=1.3][align=left] {$\rho$};
% Text Node
\draw[color={rgb, 255:red, 208; green, 2; blue, 27 }] (264,273) node [scale=1.3][align=left] {$\rho_1$};
% Text Node
\draw (160,246) node [scale=1.3][align=left] {$\rho_2$};
% Text Node
\draw (173,203) node [scale=1.3][align=left] {$\pi_1$};
% Text Node
\draw (222,136) node [scale=1.3][align=left] {$\pi_2$};
% Text Node
\draw (305,57) node [scale=1.3][align=left] {$\pi_k = \pi_{\up}$};
% Text Node
\draw (219,86) node [scale=1.3][rotate=-305] [align=left] {...};


\end{tikzpicture}


==> vass-comm.tex <==



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> vass.tex <==
% !TEX root = main.tex

\subsection{Vector addition systems}\label{vass}
In this \lcnamecref{vass}, we apply \cref{geometric-separability} to
prove \cref{result-vass-zvass}. \Cref{geometric-separability} tells us that
in order to decide whether $\sep{L}{Z_n}$ for $L\subseteq\Sigma_n^*$,
it suffices to check whether there are $k\in\N$,
$\ell_1,\ldots,\ell_m\in\N$, and vectors
$\vec u_1,\ldots,\vec u_m\in\Z^n$ such that
$L\subseteq M_k\cup D_{\vec u_1,\ell_1}\cup\cdots\cup D_{\vec
  u_m,\ell_m}$. It is tempting to conjecture that there is a finite collection of direction vectors
$F\subseteq\Z^n$ (such as a basis together with negations)
so that for a given language $L$, such an inclusion holds only if it
holds with some $\vec u_1,\ldots,\vec u_m\in F$.
In that case we would
only need to consider scalar products of words in $L$ with vectors in
$F$ and thus reformulate the problem over sections of reachability
sets of VASS. However, this is not the case. For
$\vec u,\vec v\in\Q^n$, we write $\vec u\sim\vec v$ if
$\Q_+\vec u=\Q_+\vec v$. Since $\sim$ has infinitely many equivalence
classes and every class intersects $\Z^n$, the following shows that
there is no  fixed set of directions.

\begin{restatable}{proposition}{noFixedDirections}\label{no-fixed-directions}
  For each $\vec u\in\Z^n$, there is a $k_0\in\N$ such that for
  $k\ge k_0$, the following holds.  For every
  $\ell,\ell_1\ldots,\ell_m\ge 1$, $\vec u_1,\ldots,\vec u_m\in\Z^n$
  with $\vec u_i\not\sim\vec u$ for $i\in[1,n]$, we have
  $D_{\vec u,k}\not\subseteq M_{\ell}\cup D_{\vec u_1,\ell_1}\cup\cdots
  D_{\vec u_m,\ell_m}$.
  %if and only if for some $i\in[1,m]$, we have
%  $\Q_+\vec u_i=\Q_+\vec u$ and $k\le \ell_i\|\vec u\|/\|\vec u_i\|$.
\end{restatable}

%We now turn to the VASS case.
%For $K, L\subseteq\Sigma^*_n$, we write $\modsep{L}{K}$ if for some
%$k\in\N$, we have $L\subseteq M_k$ and $M_k\cap K=\emptyset$.
%Our main goal in this section is to prove the following theorem.
%\begin{theorem}\label{thm:reduction-to-modular}
%  Given a VASS language $L$, one can construct a finite collection
%  $L_1, \ldots, L_p$ of VASS languages such that $\sep{L}{Z_n}$ if and
%  only if $\modsep{L_i}{Z_n}$ for every $i\in[1,p]$.
%\end{theorem}
%Notice that proving \cref{thm:reduction-to-modular} finishes the proof of~\cref{result-vass-zvass}.
%Indeed, checking whether $\modsep{L_i}{Z_n}$ for $i\in[1,p]$ is immediately decidable by~\cref{modular-separability}
%Thus the rest of this section is devoted to the proof of \cref{thm:reduction-to-modular}.
%
%We first define the notion of an \emph{envelope} of a language.
%Intuitively speaking it is a finite automaton, whose language contains a given language, but is not much bigger.
%For an automaton $A$ let $\Loop(A)$ be the set of all words, which label some cycle in $A$.
%For automata $A_1$ and $A_2$ and $a \in \Sigma$ the automaton $A_1 a A_2$ is created by adding an $a$-labelled
%transition from every accepting state of $A_1$ to every initial state of $A_2$.
%We say that finite automaton $A$ is an \emph{envelope} of a language $L \subseteq \Sigma_n^*$ if
%$A = A_1 a_1 A_2 \ldots A_m a_m A_{m+1}$, where $a_i \in \Sigma_n$ and $A_i$ are nondeterministic finite automata such that
%\begin{enumerate}[(1)]
%  \item $L \subseteq L(A)$\label{item:1}
%  \item for every word $w \in L$, words $u_1, \ldots, u_j \in \Loop(A)$
%  and $k \in \N$ there exist a word $w' \in L$ such that:\label{item:2}
%  \begin{enumerate}[(a)]
%    \item $\varphi(w) \equiv \varphi(w') \bmod{k}$\label{item:2a}
%    \item all the words $u_1, \ldots, u_j$ are infixes of $w'$.\label{item:2b}
%\end{enumerate}

We now turn to the proof of \cref{result-vass-zvass}. According to
\cref{geometric-separability}, we have to decide whether a given VASS
language $L\subseteq\Sigma^*_n$ satisfies
$L\subseteq M_k\cup D_{\vec u_1,\ell_1}\cup\cdots\cup D_{\vec
  u_m,\ell_m}$ for some $k\in\N$, $\vec u_1,\ldots,\vec u_m\in\Z^n$
and $\ell_1,\ldots,\ell_m\in\N$. Our algorithm employs the KLMST
decomposition used by Sacerdote and
Tenney~\cite{sacerdote1977decidability}, Mayr~\cite{DBLP:conf/stoc/Mayr81},
Kosaraju~\cite{DBLP:conf/stoc/Kosaraju82}, and
Lambert~\cite{DBLP:journals/tcs/Lambert92} and recently cast in terms
of ideal decompositions by Leroux and
Schmitz~\cite{DBLP:conf/lics/LerouxS15}. The decomposition yields VASS
languages $L_1,\ldots,L_p$ so that $L=L_1\cup\cdots\cup L_p$ so that
it suffices to check whether $L_i$ is geometrically separable for each
$i\in[1,n]$.  This is easier than for $L$, because the decomposition
also provides a structure for each $L_i$ that will guide our algorithm.

\paragraph*{Modular envelopes}
Before we dive into the KLMST decomposition, let us describe what
information it yields. We say that an automaton $\cA$ is a \emph{modular envelope}
for a language $L\subseteq\Sigma^*$ if (i)~$L\subseteq L(\cA)$ and (ii)
%\begin{enumerate}
%\item
%
% \item
  for every selection $u_1,\ldots,u_m\in\Sigma^*$ of words from
  $\Loop(\cA)$ and every $w\in L$ and every $k\in\N$, there is a word
  $w'\in L$ so that each $u_j$ is a factor of $w'$ and
  $\Parikh(w')\equiv\Parikh(w)\bmod{k}$.
%\end{enumerate}
%
  In other words, $\cA$ describes a regular overapproximation that is
  small enough that we can place every selection of loops in a word
  from $L$ whose Parikh image is congruent modulo $k$ to a given
  word. Using the KLMST decomposition, we prove:
\begin{restatable}{theorem}{constructModularEnvelopes}\label{construct-modular-envelopes}
  Given a VASS language $L$, one can construct VASS languages
  $L_1,\ldots,L_p$, together with a modular envelope $\cA_i$ for each
  $L_i$ such that $L=L_1\cup\cdots\cup L_p$.
\end{restatable}
We postpone the proof of \cref{construct-modular-envelopes} until
later and first show how
\cref{construct-modular-envelopes} can be used to decide whether $L$
is geometrically separable.

\paragraph{Modular envelopes with cone $\Q^n$} By
\cref{lem:dichotomy} we know that every cone either equals $\Q^n$ or
is included in some half-space. The following lemma will be useful in
the first case.
\begin{lemma}\label{lem:all-directions}
  Let $L\subseteq\Sigma_n^*$ be a language with a modular envelope $\cA$.  If
  $\cone(\cA) = \Q^n$ then the following are equivalent:
  (i)~$\sep{L}{Z_n}$,
  (ii)~$L \subseteq M_k$ for some $k\in\N$,
  (iii)~$\sep{\Perms(L)}{Z_n}$.
\end{lemma}
\begin{proof}
  Note that (ii) implies (iii) immediately and that (iii) implies (i)
  because $L\subseteq\Perms(L)$. Thus, we only need to show that (i)
  implies (ii).  By \cref{geometric-separability} if $\sep{L}{Z_n}$,
  then $L$ is included in some
  $M_k \cup D_{\vec u_1,k} \cup \cdots \cup D_{\vec u_m,k}$.  We show
  that in our case actually $L \subseteq M_k$.

  Take any $w \in L$. We aim at constructing $w' \in L$ such that
  $w' \notin D_{\vec u_i,k}$ for every $i \in [1,m]$ and
  additionally $\varphi(w') \equiv \varphi(w) \bmod{k}$.  Since
  $\cone(\cA) = \Q^n$, for every $\vec u_j$, there exist a loop $v_j$
  in $\cA$ such that $\scal{\varphi(v_j)}{\vec u_j} < 0$.  Since
  $\varphi(v_j),\vec u_j\in\Z^n$, we even have
  $\scal{\varphi(v_j)}{\vec u_j} \leq -1$.  Since each $v_j$ belongs
  to $\Loop(\cA)$, the words $v_j^{k+1}$ also belong to $\Loop(\cA)$.

  Since $\cA$ is a modular envelope, there exists a word $w' \in L$
  that has all the words
  $v_1^{k+1}, \ldots, v_{m}^{k+1}$ as factors and where
  $\Parikh(w) \equiv \Parikh(w') \bmod{k}$.
  Recall that every factor $u$ of every word in $D_{\vec u_i, k}$ has
  $\scal{\varphi(u)}{\vec u_j} \geq -k$. However, we have the inequality
  $\scal{\varphi(v_j^{k+1})}{\vec u_j} \leq -(k+1)$. Thus, $w'$ cannot
  belong to $D_{\vec u_i,k}$ for $i \in [1,m]$.  Since
  $L\subseteq M_k\cup D_{\vec u_1,k}\cup\cdots \cup D_{\vec u_m,k}$,
  this only leaves $w' \in M_k$. Since
  $\Parikh(w')\equiv \Parikh(w)\bmod{k}$, we also have
  $\varphi(w')\equiv\varphi(w)\bmod{k}$ and thus $w\in M_k$.
\end{proof}


% For $K, L\subseteq\Sigma^*_n$, we write $\modsep{L}{K}$ if for some
% $k\in\N$, we have $L\subseteq M_k$ and $M_k\cap K=\emptyset$.
% Our main goal in this section is to prove the following theorem.
% \begin{theorem}\label{thm:reduction-to-modular}
%   Given a VASS language $L$, one can construct a finite collection
%   $L_1, \ldots, L_p$ of VASS languages such that $\sep{L}{Z_n}$ if and
%   only if $\modsep{L_i}{Z_n}$ for every $i\in[1,p]$.
% \end{theorem}
% This would finish the proof of decidability, as \cref{thm:reduction-to-modular} 
% reduces regular separability to modular separability. The latter was already
% shown to be decidable in~\cite{}.
% \wojtek{Give more details here and write it better.}
% Thus the rest of this section is devoted to the proof of \cref{thm:reduction-to-modular}.

% We first define the notion of an \emph{envelope} of a language.
% Intuitively speaking it is a finite automaton, whose language contains a given language, but is not much bigger.
% For an automaton $A$ let $\Loop(A)$ be the set of all words, which label some cycle in $A$.
% For automata $A_1$ and $A_2$ and $a \in \Sigma$ the automaton $A_1 a A_2$ is created by adding an $a$-labelled
% transition from every accepting state of $A_1$ to every initial state of $A_2$.
% We say that finite automaton $A$ is an \emph{envelope} of a language $L \subseteq \Sigma_n^*$ if
% $A = A_1 a_1 A_2 \ldots A_m a_m A_{m+1}$, where $a_i \in \Sigma_n$ and $A_i$ are nondeterministic finite automata such that
% \begin{enumerate}[(1)]
%   \item $L \subseteq L(A)$\label{item:1}
%   \item for every word $w \in L$, words $u_1, \ldots, u_j \in \Loop(A)$
%   and $k \in \N$ there exist a word $w' \in L$ such that:\label{item:2}
%   \begin{enumerate}[(a)]
%     \item $\varphi(w) \equiv \varphi(w') \bmod{k}$\label{item:2a}
%     \item all the words $u_1, \ldots, u_j$ are infixes of $w'$.\label{item:2b}
%   \end{enumerate}
% \end{enumerate}

% Notice that not every language has an envelope, for example $\{a, b\}$ does not have.
% However, VASS languages exhibit a special behavior in this respect, as stated by the following lemma.

% \begin{lemma}\label{lem:decomposition}
% For every VASS language $L$ one can compute finitely many VASS languages $L_1, \ldots, L_r$ such
% that $L = \bigcup_{i=1}^r L_i$ and every $L_i$ has an envelope.
% \end{lemma}

% We prove \cref{lem:decomposition} in \cref{sec:decomposition-proof}.


\begin{algorithm}
  \DontPrintSemicolon
  \SetKwInOut{Input}{Input}
  \SetKw{Exit}{exit}
  \Input{$n\in\N$ and VASS language $L=\Lang{V}\subseteq\Sigma_n^*$}
  \caption{Deciding separability of a VASS language $L$ from $Z_n$}\label{algorithm}

  \lIf{$n=0$ and $L=\emptyset$}{\Return{``yes''}}
  \lIf{$n=0$ and $L\neq \emptyset$}{\Return{``no''}}
  Use KLMST decomposition to compute VASS languages $L_1,\ldots,L_p$,
  together with modular envelopes $\cA_1,\ldots,\cA_p$.\\
  \For{$i\in[1,p]$}{
    \If{$\cone(\cA_i)=\Q^n$}{
      Check whether $\Perms(L_i)|Z_n$\\
      \lIf{not $\Perms(L_i)|Z_n$}{
        \Return{``no''}
      }
    }
    \If{$\cone(\cA_i)\subseteq H=\{\vec x\in\Q^n\mid \langle \vec x,\vec u\rangle\ge 0\}$ for some $\vec u\in\Z^n\setminus \{0\}$}{
      Let $U=\{\vec x\in \Q^n\mid \langle \vec x,\vec u\rangle=0\}$. \tcc*[f]{$\dim U=n-1$} \\
      Compute $k,\ell\in\N$ with $L_i \subseteq\Lang{\cA_i}\subseteq D_{\vec u,k}\cup S_{U,\ell}$
      \tcc*[f]{$L_i\setminus D_{\vec u,k}\subseteq S_{U,\ell}$}\\
      Compute rational transduction $T_{U,\ell}\subseteq \Sigma_n^*\times\Sigma_{n-1}^*$ \\
      Check recursively whether $T_{U,\ell} (L_i\!\setminus\! D_{\vec u,k})|Z_{n-1}$ 
      \tcc*[f]{$T_{U,\ell} (L_i\!\setminus\! D_{\vec u,k})\subseteq\Sigma^*_{n-1}$}\\
      \lIf{not $T_{U,\ell} (L_i\setminus D_{\vec u,k})|Z_{n-1}$}{
        \Return{``no''}
      }
    }
  }
  \Return{``yes''}
  
\end{algorithm}

We are now prepared to explain the decision procedure for
\cref{result-vass-zvass}. The algorithm is illustrated in
\cref{algorithm}.  If $n=0$, then $\Sigma_n=\emptyset$ and thus either
$L=\emptyset$ or $L=\{\varepsilon\}$, meaning $\sep{L}{Z_0}$ if and
only if $L\ne\emptyset$.  Otherwise, we perform the KLMST
decomposition, which, as explained in the next section, yields
languages $L_1\cup\cdots\cup L_p$ and modular envelopes
$\cA_1,\ldots,\cA_p$ such that $L=L_1\cup\cdots\cup L_n$. Since then
$\sep{L}{Z_n}$ if and and only if $\sep{L_i}{Z_n}$ for each
$i\in[1,p]$, we check for the latter. For each $i\in[1,p]$, the
dichotomy of \cref{lem:dichotomy} guides a case distinction: If
$\cone(\cA_i)=\Q^n$, then we know from \cref{lem:all-directions} that
$\sep{L_i}{Z_n}$ if and only if $\sep{\Perms(L_i)}{Z_n}$, which can be
checked via \cref{separability-commutative}.

If, however, $\cone(\cA_i)$ is contained in some half-space
$H=\{\vec x\in\Q^n \mid \langle x,\vec u\rangle\ge 0\}$ for some
$\vec u\in\Z^n$, then \cref{halfspace} tells us that
$L_i\subseteq \Lang{\cA_i}\subseteq D_{\vec u,k}\cup S_{U,\ell}$ for
some computable $k,\ell\in\N$ and
$U=\{\vec x\in\Q^n \mid \langle \vec x,\vec u\rangle=0\}$.  In
particular, we have $\sep{L_i}{Z_n}$ if and only if
$\sep{L_i\!\setminus\! D_{\vec u,k}}{Z_n}$.  Note that
$L_i\setminus D_{\vec u,k}=L\cap (\Sigma^*_n\setminus D_{\vec u,k})$
is a VASS language and is included in $S_{U,\ell}$.  Thus, the walks
corresponding to the words in $L_i$ always stay close to the
hyperplane $U$, which has dimension $n-1$. We can therefore use the
transduction $T_{U,\ell}$ to transform $L_i$ into a set of walks in
$(n-1)$-dimensional space and decide separability recursively for the
result: We have $T_{U,\ell}L_i\subseteq\Sigma_{n-1}^*$ and
\cref{dimension-reduction} tells us that $\sep{L_i}{Z_n}$ if and only if
$\sep{T_{U,\ell}L_i}{Z_{n-1}}$.


\paragraph{Constructing modular envelopes} As mentioned above, we
use the KLMST decomposition (so named by Leroux and
Schmitz~\cite{DBLP:conf/lics/LerouxS15} after its inventors
Mayr~\cite{DBLP:conf/stoc/Mayr81},
Kosaraju~\cite{DBLP:conf/stoc/Kosaraju82},
Lambert~\cite{DBLP:journals/tcs/Lambert92} and Sacerdote and
Tenney~\cite{sacerdote1977decidability}) to construct the
decomposition of $L$ into $L_1,\ldots,L_p$ with modular envelopes
$\cA_1,\ldots,\cA_p$. This decomposition is relatively unwieldy in
terms of required concepts and terminology. Moreover, the construction
of modular envelopes is not the main innovation of this paper but in
large part a combination of existing methods. Therefore, we decided to
include only a very high-level overview and keep the details in the
appendix.

The decomposition yields perfect marked graph-transition sequences
(MGTS) $\Ncal_1,\ldots,\Ncal_p$. Each MGTS $\Ncal_i$ defines a
VASS language $L_i$ so that $L=L_1\cup\cdots\cup L_p$. The MGTS are
readily translated into finite automata $\cA_1,\ldots,\cA_p$ for which
it is known that $\Lang{\cA_i}$ overapproximates
$L_i$~\cite{DBLP:conf/icalp/CzerwinskiHZ18}. For the second property
of modular envelopes, we use a concept of \emph{run amalgamations} as
introduced by Leroux and Schmitz~\cite{DBLP:conf/lics/LerouxS15}. It
permits the amalgamation of two runs into which a third run embeds via
the order $\unlhd$ on runs introduced by
Jan\v{c}ar~\cite{DBLP:journals/tcs/Jancar90} and
Leroux~\cite{DBLP:conf/popl/Leroux11}.

Given a word $w\in L_i$ and $u_1,\ldots,u_m\in\Loop(\cA)$, we use
Lambert's pumping lemma~\cite{DBLP:journals/tcs/Lambert92} to
construct a run $\rho_1$ in $\Ncal_i$ that contains $u_1,\ldots,u_m$
as factors, but that also embeds the run $\rho$ for $w$.  We argue
that this embedding has a special property that guarantees that
amalgamating $\rho$ and $\rho_1$ yields a run in $\Ncal_i$ that still
embeds $\rho$ with this property and still contains the $u_i$ as
factors. We can then repeat this process $(k-1)$-fold to obtain a run
$\rho_k$ reading a word $w_k$ where
$\Parikh(w_k)=k\cdot (\Parikh(w_1)-\Parikh(w))+\Parikh(w)$ and thus
$\Parikh(w_k)\equiv\Parikh(w)\bmod{k}$.





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

